Next-Step Hint Generation for Introductory Programming Using Large Language Models

Large Language Models possess skills such as answering questions, writing essays or solving programming exercises. Since these models are easily accessible, researchers have investigated their capabilities and risks for programming education. This work explores how LLMs can contribute to programming education by supporting students with automated next-step hints. We investigate prompt practices that lead to effective next-step hints and use these insights to build our StAP-tutor. We evaluate this tutor by conducting an experiment with students, and performing expert assessments. Our findings show that most LLM-generated feedback messages describe one specific next step and are personalised to the student's code and approach. However, the hints may contain misleading information and lack sufficient detail when students approach the end of the assignment. This work demonstrates the potential for LLM-generated feedback, but further research is required to explore its practical implementation.

==> Chapters/old/2.1_effective_theory.tex <==
\chapter{Related work}

\section{Providing Effective Feedback}\label{lit:effb}
Feedback is considered essential in the process of learning \cite{hattie2007power}. Feedback can enhance learning by correcting misconceptions or mistakes. In addition, feedback can improve the students' motivation by providing positive comments or guidance when the student is stuck. All feedback that consists of information or learning activities that support and facilitate student learning is classified as formative feedback \cite{irons2021enhancing}. Its counterpart, summative feedback, consists of assessment activities, resulting in grades that evaluate the student's performance. 

Various variables impact the effectiveness of formative feedback, such as its complexity \cite{shute2008focus}. Complexity relates to giving elaborate or concise feedback. Elaborated feedback helps students understand why something is wrong and can guide students in the right direction through explanations or tips. As a counterpart, if feedback is too long, many learners will not pay attention to it, rendering it useless. Another essential factor is timing. Feedback can be provided by intervening or waiting: until the student requests feedback themselves or finishes an assignment. Another variable of feedback is its nature, which can be positive or negative. In contrast with negative feedback, positive feedback reinforces what students are doing well, for example, to emphasise the student is correctly implementing assignment requirements. Both can, however, have beneficial effects on learning \cite{hattie2007power}.

Although many studies on effective feedback exist, defining effective feedback remains complicated due to its many aspects, such as specificity goal orientation, in addition to the previously mentioned factors \cite{shute2008focus}. Besides, even students and teachers have different ideas about what feedback is effective. Dawson \etal performed a qualitative study of teachers' and students' ideas and opinions of effective feedback \cite{dawson2019makes}. Although teachers and students agree that the overall purpose of feedback should improve student performance, they have other beliefs on what makes feedback effective. While teachers believe in the importance of timing, modalities and connected tasks, students prefer high-quality feedback comments that make feedback effective. These comments should be detailed and personalised to the student's work. Wisniewski \etal found that feedback is more effective when it contains more information \cite{wisniewski2020power}, which could correspond to the student's preference for more detailed feedback. Their work shows that simple reinforcement and punishment have slight effects, while high-information feedback is the most helpful.









==> Chapters/old/results.tex <==
% \chapter{Results}

% \section{Prompt Engineering}
% \subsection{Instructions}
% We started with three different instruction phrasings, shown in table \ref{X} with corresponding hints. As we had no idea of effective prompts for hint generation, we first wanted to obtain an initial idea of how phrasing would affect the generated hints. For this part, we did an explorative round where we noted our findings.

% As illustrated in table \ref{X}, the prompt instructions generated output with the same subject but expressed differently. Furthermore, when they had different topics, we did not discover a distinctive pattern in what cases they had other subjects. In almost all cases, the generated outputs contained information on how to proceed, which was our starting point. 

% Accordingly, we analysed the results for three phrasings. We noticed specific patterns for each instruction and summarised these findings in table \ref{X}. The prompt instructions had only slight variations among each other, consisting of a few different words. However, the generated feedback had notably different results, especially regarding additional information and phrasing of the hints. The prompt: "What is the next step?", often contained code, compared to the other two prompts. In addition, the phrasing was a bit more straightforward and blunt. 

% Contrarily, “Explain the next step for a student” resulted in relatively longer hints while sometimes also explaining the student's code. The phrasing of the feedback generated with this prompt was similar to “Give a hint for the next step”. We decided to further the prompt engineering by combining keywords from the last two prompts since we did not want the hints to contain code. 

% \subsection{Prompt templates}
% We simultaneously analysed the effect of adding different prompt attributes. We found that the best option was to include only the problem description. The prompt templates without description and model solution led to guessing from the model. For example: "The next step likely involves performing some mathematical operation using the values assigned to v2, v3, and v4". Here, the model attempted the provide a hint without addressing the overall purpose of the code or the assignment. However, as the student proceeded, the model became incapable of generating something sensible. 

% Including one of the two candidate attributes created next-step hints more related to the student code and assignment. However, the templates with a model solution often caused the model to advise students to compare their code to the model solution. This happened after editing the prompts and explicitly commanding the model not to refer to the solution. In addition, the model seemed unable to connect variables from the description or model solution to the student code. As a result, hints contained suggestions for operations the student had already implemented but used different variable names than those provided in the assignment. In addition, the feedback often centred around following the approach from the model solution even when students maintained another (allowed and correct) method. A frequently observed example was a suggestion for adding loops when the student is using join operations in the brackets exercise.

% \subsection{Temperature}\drft{
% First, we explored different temperatures for the “Give a hint for the next step” instruction (values 0.1, 0.3, 0.5, 0.7, and 0.9). We did this for this prompt with both a description and a description + model solution. To see if it would change the problem encountered before (it did not, so we chose to continue only with the description prompt. Second, we tried different variations for the prompt “Give this student a short hint for the next step” (without short, the hints were too long). To see how temperature changes would affect generated hints with different prompts. The focus of this exploring phase is to look at the differences between the different values for temperature. And see if we can find notable differences. Furthermore, we would like to see if we can find an optimal temperature.}

% We found that changing the temperature changes some things but did not cause entirely new responses. Overall, comparing the hints for per student program, we found that too high temperature caused odd suggestions. Depending on the prompt, a higher temperature causes more variation in phrasing. It seems that a longer more complex prompt will evoke this behaviour by itself.

% \section{Student Experiment}
% Figure \ref{fig:numberhints} reports the number of hints each student requested and rated during the experiment, which sums up to 48 hints. Examining the student's responses to the hint ratings, shown in Figure \ref{fig:ratings} \note{weglaten?}, we notice the students marked the hints as clear and fitted to their work. The students were less convinced about the usefulness of the feedback as they labelled hints helpful only half of the time \note{uitbreiden over usefulness, misschien comments tijdens het experiment}, while not one student finished the assignment in the provided time frame. Even though all students believed that the exercise corresponded with their current skills and programming level, not one student had a correct solution at the end of the experiment. The students had especially trouble with the logic for correctly counting the clumps, which required tracking and implementing when to "count" a clump with conditional statements.  

% \begin{figure}[h!]
%     \begin{minipage}{0.49\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/numberofhintsperstudent.pdf}
%         \caption{Rated hints per student}
%         \label{fig:numberhints}
%     \end{minipage}
%     \begin{minipage}{0.49\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/allstudentratingsperquestion.pdf}
%         \caption{Student ratings per question}
%         \label{fig:ratings}
%     \end{minipage}
% \end{figure}

% \subsection{Overall students' impression}
% After the experiment, we asked the students several final questions about their experiences and opinions. Overall, they had a positive impression of the StAP-tutor and appreciated the hints, especially at the beginning of the experiment. The students found that at the start of the assignment, the hints fit the student's work and had practical suggestions for what to do next. However, after a while, when the student was stuck with more complex code, the hints were not helpful anymore. In those cases, the students stated they needed more detail, and the hints remained too vague. In addition, the students indicated they found it difficult to program without additional information a standard IDE provides, such as simple syntax errors or the ability to run their code. 

% We found it remarkable that all students mentioned using the StAP-tutor to request multiple hints for the same code. As the language model is not deterministic, it might help to regenerate a hint when it is too vague or not necessarily helpful. They noted that regenerating creates a different phrasing or provides more or new information. However, one of the students stated that requesting the same hints for the same code could even be more helpful if those hints entail more details. 

% Compared to ChatGPT, the StAP-tutor focuses more on your existing code rather than providing a general solution with much additional information. The student thought this might help with learning as this also reduces the temptation to copy and paste the assignment and generate a whole solution. However, as one of the students points out, an advantage of ChatGPT is that there is a possibility to ask more specific questions yourself. The StAP-tutor uses automatically generates the prompts and has no opportunity for student input. 

% \section{Expert Assessment}
% \drft{
% We started our expert evaluation by coordinating our interpretations of the evaluation criteria. We first did this for a set of 6 hints and than both rated a randomly selected set of 19 hints. For this subset, we compared our answers for which the agreements are shown in table \ref{table:reliability}. Additionally, we computed the corresponding inter-rater reliability with Cohen's Kappa. According to a proposed interpretation from Landis \etal, we interpret values from 0.21-0.40 as Fair, 0.41-0.60 as "Moderate", 0.61-0.80 "Substantial" and 0.81-1.00 as "Almost Perfect" \cite{landis1977measurement}. The experts had low agreement for level-of-detail and tone, which was expected as the tone is presumably a relatively subjective category. In addition. We consider overall that we have a sufficient substantial agreement between the two experts. We made sure to have an agreement discuss the disagreements, came to an agreement and merged these ratings with the remaining 29 ratings, performed by only the author of this work. We demonstrated our agreement and assume that the rating the remaining hints individually will be in line with our other ratings. 
% }

% \begin{table}[h!]
% \caption{Inter-rater reliability for the expert evaluation}
% \begin{tabularx}{\linewidth}{lXXXX}
% \hline
%                         & \textbf{Feedback Type} & \textbf{Information} & \textbf{Level-of-detail} & \textbf{Personalized} \\ \hline
% \textit{Agreements} &  22/22                      & 21/22                    & 19/22                        & 21/22                     \\
% \textit{Cohen’s kappa}           & 0.765                  & 0.787               & 0.387                    & 0.883                 \\
%                         &                        &                      &                          &                       \\ \hline
%                         & \textbf{Appropriate}            & \textbf{Specific}             & \textbf{Misleading Information }  & \textbf{Tone}              \\ \hline
% \textit{Agreements} & 21/22                     & 21/22                    & 20/22                        & 18/22                     \\
% \textit{Cohen’s kappa  }         & 0.855                  & 0.642                & 0.683                    & 0.467            \\ \hline    
% \end{tabularx}
% \label{table:reliability}
% \end{table}

% \drft{
% Looking at the figures presented below, we see the frequencies for the criteria "Feedback Type, \textit{Level-of-detail} and "Tone". The majority of the generated hints correspond to \textit{Knowledge About How To Proceed}, which is ultimately the main focus of this work. Moreover, the hints are more high-level hints. Note, in contrast with the type of feedback, we did not particularly specify in the prompt the level of detail we desired. Still, the model had a tendency for these prompt settings for generating more high-level hints. Finally, we found that most feedback was most of the time friendly.  
% }

% \begin{figure}[h!]
%   \centering
%   \begin{minipage}[t]{0.30\textwidth}
%     \includegraphics[width=\linewidth]{figures/Feedback Type.pdf}
%     \caption{Feedback Type}
%     \label{fig:fbtyp}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[t]{0.30\textwidth}
%     \includegraphics[width=\linewidth]{figures/Level-of-detail.pdf}
%     \caption{Level of detail}
%     \label{fig:level}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[t]{0.30\textwidth}
%     \includegraphics[width=\linewidth]{figures/Phrasing.pdf}
%     \caption{Tone}
%     \label{fig:phrasing}
%   \end{minipage}
%   \hfill
% \end{figure}

% \drft{
% We found that being friendly correlates with hints containing additional information. Naturally, when a hint states "Keep up the good work!", we interpret this as friendly or kind. In Figure \ref{fig:information}, we see the number of occurrences for every category of additional information. We occasionally saw smaller tips in addition to the "main" hint. These tips would often refer to something that was the student not yet working on. For example "Also, try to think about the conditions under which a clump exists." or "Don't forget to handle the cases where the clump ends or a new clump begins". 
% }

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.7\textwidth]{figures/information.pdf}
%     \caption{Caption}
%     \label{fig:information}
% \end{figure}

% \drft{
% All evaluation metrics with binary values are presented in Figure \ref{fig:binaryeval}. Misleading information: verkeerde reden waaorm iets gebeurt (The for loop of your current code may reach an out-of-range index error if it reaches the end of the list without finding a clump.) waarom iets fout is of hoe iets gedaan moet worden. Soms suggereert het iets, maar dat zal het probleem niet oplossen is niet nodig (You need to make sure your program doesn't break when the input array has only one element.) Notably, misleading information is often linked to hints that refer to edge cases (first/last clumps etc). 
% }

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.8\textwidth]{figures/Binary Eval.pdf}
%     \caption{Frequencies of binary evaluation metrics: Personalised, Appropriate, Specific and Misleading Information}
%     \label{fig:binaryeval}
% \end{figure}



==> store.tex <==
% \begin{enumerate}
%     \item Within the context of teaching programming to novices, Corbett and Anderson showed that for formative feedback to be most effective for programming students, it has to be immediate and point to individual steps and features in the learner’s work.
%     \item  Second, introducing problem-solving concepts before teaching more specific programming aspects has an impact on how students learn to program. This strategy could help students realize that it is essential to develop an ability to both break down complex problems into subtasks and produce the correct sequence of actions and accelerate consolidation of concepts, such as data and control structures, introduced later in the course. From this perspective, programming problems can then be solved as a systematic implementation of tackling one sub task at a time and back- tracking afterwards. \cite{koulouri2014teaching}
%     \item Finally, specifically for novice programmers, Rivers found that less experienced programmers wanted more detailed content in their hints, compared with more experienced programmers, and that most users wanted hints to give as little information as possible, while allowing the option to see more detail if necessary. \cite{rivers2017data}
%     \item Setting up the evaluation of intelligent tutoring systems is a complex task \cite{beck2008does}, and unfortunately, several studies report on the lack of evaluation for the development of automated feedback. Ideally, to assess the effectiveness of feedback, one would analyse the student learning performance between two student groups over a significant amount of time in which the group is allowed feedback. However, reality often does not allow for such extensive evaluation. Furthermore, providing feedback to only a subset of all students can raise ethical concerns about exclusion and fairness.
% \end{enumerate}
